SimWorld: An Open-ended Realistic Simulator for Autonomous Agents in Physical and Social Worlds

While LLM/VLM-powered AI agents have advanced rapidly in math, coding, and computer use, their applications in complex physical and social environments remain challenging. Building agents that can survive and thrive in the real world (for example, by autonomously earning income or running a business) requires massive-scale interaction, reasoning, training, and evaluation across diverse embodied scenarios. However, existing world simulators for such development fall short: they often rely on limited hand-crafted environments, simulate simplified game-like physics and social rules, and lack native support for LLM/VLM agents. We introduce SimWorld, a new simulator built on Unreal Engine 5, designed for developing and evaluating LLM/VLM agents in rich, real-world-like settings. SimWorld offers three core capabilities: (1) realistic, open-ended world simulation, including accurate physical and social dynamics and language-driven procedural environment generation; (2) a rich interface for LLM/VLM agents, with multimodal world inputs and open-vocabulary actions at varying levels of abstraction; and (3) diverse and extensible physical and social reasoning scenarios that are easily customizable by users. We demonstrate SimWorld by deploying frontier LLM agents (e.g., GPT-4o, Gemini-2.5-Flash, Claude-3.5, and DeepSeek-Prover-V2) on long-horizon multi-agent delivery tasks involving strategic cooperation and competition. The results reveal distinct reasoning patterns and limitations across models. We open-source SimWorld and hope it becomes a foundational platform for advancing real-world agent intelligence across disciplines: https://simworld.org.

==> configs/header.tex <==
% Define and set date
\makeatletter
\def\icmldate#1{\gdef\@icmldate{#1}}
\icmldate{Technical Report} %. Release Date: \today}
\makeatother

% Define page style
\makeatletter
\fancypagestyle{fancytitlepage}{
  \fancyhead{}  % clear all headers
  % \lhead{\includegraphics[height=0.75cm]{figures/logos/maitrix.png}}
  % \lhead{\includegraphics[height=0.75cm]{figures/logos/simworld.jpg}}
  \rhead{\it \@icmldate}
  \cfoot{}
}
\makeatother

==> floating/algorithms/embodied_multi_agent_task_generation.tex <==
\begin{algorithm}[H]
\caption{Task Generation for Multi-robot Search}
\KwIn{City map with $m$ streets; sample $n$ landmark buildings per street}
\KwOut{main robot's memory $\mathcal{M}$, main robot spawn $s_{\text{main}}$, following robot spawn $s_{\text{follow}}$}

\tcp{Phase 1: Build Main Robot’s Memory}
Initialize memory set $\mathcal{M} \leftarrow [\,]$\;

\For{$i \leftarrow 1$ \KwTo $m$}{
    Sample $n$ landmark buildings on street $i$: $\{L_{i1}, L_{i2}, \dots, L_{in}\}$\;

    \For{$j \leftarrow 1$ \KwTo $n$}{
        $x_{ij} \leftarrow$ get front-door location of $L_{ij}$\;

        $o_{ij} \leftarrow$ compute orientation facing toward $L_{ij}$\;

        $I_{ij} \leftarrow$ capture visual cue at $x_{ij}$ with orientation $o_{ij}$\;

        Add $(I_{ij}, x_{ij})$ to memory set $\mathcal{M}$\;
    }
}

\tcp{Phase 2: Sample Initial Robot Positions}
Obtain a set of valid robot spawn points $S$\;

Randomly sample two distinct spawn points from $S$: $s_{\text{main}}, s_{\text{follow}}$\;

\Return $(\mathcal{M}, s_{\text{main}}, s_{\text{follow}})$
\label{alg:mrs-task-gen}
\end{algorithm}

==> floating/algorithms/embodied_single_agent_task_generation.tex <==
\begin{algorithm}[H]
\caption{Task Generation for Multi-modal Robot Navigation}
\KwIn{Navigation path $P = \{n_1, n_2, \dots, n_k\}$, orientations $\{\theta_1, \theta_2, \dots, \theta_k\}$}
\KwOut{Ordered list of subtasks $\mathcal{T} = \{(I_1, V_1), (I_2, V_2), \dots\}$}

Initialize subtask list $\mathcal{T} \leftarrow [\,]$\;

$V_1 \leftarrow$ capture visual cue at $n_1$ with orientation $\theta_1$\;

$I_1 \leftarrow$ generate \textbf{Orientation Alignment} instruction using compass heading $\theta_1$ and nearby landmark\;

Add $(I_1, V_1)$ to $\mathcal{T}$\;

\For{$i \leftarrow 2$ \KwTo $k-1$}{
    \If{$\theta_i \neq \theta_{i-1}$}{
        $V_\text{move} \leftarrow$ capture visual cue at $n_{i-1}$ with orientation $\theta_{i-1}$\;
        
        $I_\text{move} \leftarrow$ generate \textbf{Move Along the Road} instruction using a landmark near $n_{i-1}$\;

        Add $(I_\text{move}, V_\text{move})$ to $\mathcal{T}$\;

        $V_\text{turn} \leftarrow$ capture visual cue at $n_i$ with new orientation $\theta_i$\;

        $I_\text{turn} \leftarrow$ generate \textbf{Turn at Intersection} instruction based on the relative angle between $\theta_{i-1}$ and $\theta_i$\;

        Add $(I_\text{turn}, V_\text{turn})$ to $\mathcal{T}$\;
    }
}

$V_\text{goal} \leftarrow$ capture visual cue at $n_k$ with orientation $\theta_k$\;

$I_\text{goal} \leftarrow$ generate \textbf{Reach Destination} instruction using goal landmark description\;

Add $(I_\text{goal}, V_\text{goal})$ to $\mathcal{T}$\;

\Return $\mathcal{T}$
\label{alg:mmnav-task-gen} 
\end{algorithm}

==> floating/images/assets.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/assets.pdf}
    \vspace{-16pt}
    \caption{A subset of the asset collection in UE.}
    \label{fig:assets} 
\end{figure}

==> floating/images/asynchronized.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/asynchronized.pdf}
    \caption{\textbf{Asynchronized multi-agent control.} To ensure each agent independently selects and executes actions based on its local observation and policy model, a centralized buffer serves as the interface between agents and the environment, receiving actions from all agents and updating their observations based on the resulting environmental changes.}
    \label{fig:asynchronized}
\end{figure}

==> floating/images/layout.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/CLPG.pdf}
    \caption{\textbf{Generation Pipeline for Static World Initialization.} The process consists of four stages: (1) road network generation, (2) procedural building placement and (3) insertion of street-level elements.}
    \label{fig:clpg}
\end{figure}

==> floating/images/maps.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/map_categories_histogram.pdf}
    \caption{The statistical distribution of environments in \simworld.}
    \label{fig:maps}
\end{figure}

==> floating/images/observation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/observation.pdf}
    \caption{\textbf{Observation space of SimWorld Agent.} From left to right: RGB, segmentation, and depth.}
    \label{fig:observation_space}
\end{figure}

==> floating/images/physical_choice_proportion.tex <==
\begin{figure}[ht]
  \centering
  \begin{minipage}[t]{\textwidth}
    \centering
    \begin{minipage}[t]{0.3\textwidth}
      \includegraphics[width=\linewidth]{figures/physical/model_comparison_bar_success_normal.pdf}
      \centering
      \scriptsize (a) Comparison of model action types in static obstacle environments (success cases analysis).
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.3\textwidth}
      \includegraphics[width=\linewidth]{figures/physical/model_comparison_bar_success_ped.pdf}
      \centering
      \scriptsize (b) Comparison of model action types in dynamic obstacle (pedestrian) environments (success cases analysis).
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.3\textwidth}
      \includegraphics[width=\linewidth]{figures/physical/model_comparison_bar_all_non.pdf}
      \centering
      \scriptsize (c) Comparison of model action types without local action planner (all cases analysis).
    \end{minipage}

    \vspace{0.5em}
    \caption{\textbf{Distribution of Action Types for Navigation Models in Environments with/without Obstacles and Different Obstacle Types.}}
    \label{fig:llm_choice_proportion}
  \end{minipage}
\end{figure}


==> floating/images/physical_distance.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/physical/combined_distance_to_goal.pdf}
    \caption{\textbf{Step-wise Average Destination Distance across Tasks.} \texttt{GPT-4o} often exhibits early stagnation, making limited goal progress, while \texttt{Claude-3.7-Sonnet} shows fluctuating effectiveness. \texttt{Gemini-2.5-Pro} stands out by demonstrating the most stable and continuous reduction in goal distance, highlighting its superior planning and navigation capabilities without a local action planner.}
    \label{fig:combined-distance}
\end{figure}



==> floating/images/realistic.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/realistic&agent.pdf}
    \caption{Realistic Environments and Rich Embodied Agents.}
    \label{fig:realistic}
\end{figure}

==> floating/images/traffic.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/traffic.pdf}
    \caption{Traffic system.}
    \label{fig:traffic}
\end{figure}

==> floating/images/waypoint.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/waypoint.pdf}
    \caption{Waypoint System and Action Planner.}
    \label{fig:waypoint}
\end{figure}

==> floating/tables/delivery_actionspace.tex <==
\begin{table}[th]
    \centering
    \caption{\textbf{Hierarchical Action Space Design in Agent Social Reasoning Experiment.} High-level actions are given to language models to make decision, which correspond to strategic decisions, while low-level actions are only exposed to local action planner module to execute concrete movements and interactions.}
    \label{tab:delivery-action-space}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{llll}
        \toprule
        \textbf{Action Level} & \textbf{Action Name} & \textbf{Description} &\textbf{Invocation Method} \\
        \midrule
        \multirow{9}{*}{High-Level Actions} 
            & Bid Order & Offer a price to a new order on platform to compete with other Model Generations & Model Generation \\
            & Pick Up Order & Navigate to the pick-up point of order & Model Generation\\
            & Deliver Order & Navigate to the delivery point and complete the order & Model Generation \\
            & Share Order & Publish the order for multi-model generation cooperation & Model Generation \\
            & Cancel Share Order & Cancel a shared order that has been published & Model Generation \\
            & Go to Meet-point & Navigate to the meet point for the shared order & Model Generation \\
            & Purchase Scooter & Buy and use a scooter & Model Generation \\
            & Purchase Drinks & Buy consumables to restore energy & Model Generation \\
            & Adjust Speed & Adjust travel speed & Model Generation \\
        \midrule
        \multirow{5}{*}{Low-Level Actions}
            & Move Forward & Basic movement action & Local Planner \\
            & Stop & Stop moving & Local Planner\\
            & Rotate & Adjust the facing direction &  Local Planner  \\
            & Change Speed & Adjust walking speed & Local Planner \\
            & Drive Scooter & Control a scooter for movement & Local Planner \\
            % & Pick Up & Execute pick-up animation and interaction &  Local Planner \\
            % & Drop Off & Execute delivery action &  Local Planner\\
            % & Get on Scooter & Mount the scooter to change movement mode & Local Planner \\
            % & Interact & Trigger contextual interactions (e.g., purchasing drinks) & A2A module / Model Generation direct \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> sections/04-agent-interface.tex <==
\input{floating/images/userstory}
\section{Agent Interface}
\subsection{Controlling Embodied Agents (New)}
% \subsection{Task Suite Creation Workflow}

\simworld supports three types of embodied agents—humans, vehicles, and robots. Unlike synchronized designs~\cite{puig2018virtualhomesimulatinghouseholdactivities} where agents must wait for others to complete their actions, \simworld allows asynchronous control, enabling each agent to act independently. To better reflect real-world conditions and support diverse tasks, \simworld also provides rich action spaces for different agents and flexible observation spaces.

\textbf{Types of Embodied Agents.} Unlike previous simulators~\cite{Dosovitskiy17, wu2025metaurban, li2022metadrive} that focus on a specific type of embodied agent---such as autonomous vehicles, robots, or humans---and mainly support control over that particular agent type, our simulator simultaneously supports all three major categories. This unified design enables the development of broader and more diverse embodied AI tasks within a single environment. 

\textbf{Asynchronized Multi-agent Control.} To realistically model scenarios where multiple agents act independently and simultaneously, \simworld uses an asynchronous multi-agent control framework. Each agent receives its observation from a centralized buffer and can submit an action only when marked as available. The buffer updates at a fixed interval (default: 0.01 seconds), checking for actions from available agents and updating their availability status. Valid actions are executed concurrently, after which all agents become unavailable until their actions complete. Once finished, agents are marked as available again and receive updated observations.

\textbf{Observation Space.} \simworld provides three primary types of visual observations: RGB images, depth images, and semantic segmentation masks. In addition to these, \simworld also offers ground-truth language descriptions and 3D bounding boxes for objects present in the environment.

% \input{floating/images/observation}

\textbf{Action Space.} \simworld provides a rich and versatile action space tailored to different types of agents. For vehicles: acceleration, braking, and steering. Each action is continuous within a set range, allowing flexible control—e.g., higher acceleration leads to faster speeds, and larger steering values result in sharper turns. For robot control, actions include continuous translation (forward, backward, left, right) and free-angle rotation, enabling flexible movement and orientation. Human agents can perform typical navigation actions (movement, turning) and a set of interaction actions relevant to urban scenarios, grouped into: (1) human–object (e.g., pick up/drop off objects, sit/stand), (2) human–vehicle (e.g., drive, enter/exit, open/close trunk), and (3) human–human (e.g., wave, argue, point). Table~\ref{tab:simworld-actionspace-full} provides a full list of action space.

\input{floating/tables/actionspace}

\subsection{Connecting \simworld to LLM/VLMs (New)}

\simworld is designed to make the deployment of LLM/VLM agents straightforward and flexible by exposing a rich, modular input-output interface. This design supports diverse forms of evaluation, reasoning, and training for agents operating in complex environments.

For an agent's inputs, \simworld supports both raw sensor data (RGB, depth, segmentation) and symbolic representations (semantic graphs, event-based feedback). This multi-level design enables LLM/VLM agents to operate at different abstraction levels, from low-level perception to high-level reasoning.

For an agent's outputs, \simworld moves beyond the restrictive, low-level action spaces of many existing simulators (e.g., “move forward by 1 block” in Minecraft). It provides a dual-layer control interface: agents can issue primitive low-level actions (e.g., throttle, step forward, picking up an object) for fine-grained control, or express high-level natural language commands (e.g., \textit{"go to the nearest chair and sit down"}). A built-in {\bf local action planner} interprets these high-level commands and decomposes them into executable primitive actions.

% For an agent's outputs, \simworld moves beyond the restrictive, low-level action spaces of many existing simulators (e.g., “move forward by 1 block” in Minecraft). Instead, \simworld supports an open-vocabulary action interface that accepts natural language commands at varying levels of abstraction. For instance, an agent can issue a high-level instruction such as ``\texttt{go to the nearest chair and sit down}''. A built-in {\bf local action planner} interprets this instruction and decomposes it into a sequence of low-level actions executable by the simulator (see Section~\ref{sec:local-action-planner}).

This dual design allows agents to flexibly choose the most suitable level of control depending on the task: leveraging high-level abstraction for long-horizon reasoning, while retaining the option of low-level embodiment when precision is required. As a result, \simworld bridges the gap between cognition and embodiment, making it a practical and extensible platform for building and evaluating intelligent agents.

% This layered design enables LLM/VLM agents to focus on long-horizon reasoning and high-level decision-making, while offloading low-level physical execution to the simulator. As a result, \simworld bridges the gap between high-level cognition and low-level embodiment, making it a practical and extensible platform for building and evaluating intelligent agents.

\subsubsection{Local Action Planner (NeurIPS Appendix)}
\label{sec:local-action-planner}

\simworld integrates an action planning module within the simulator, aligning with recent advances in agent architectures and providing LLM agents with a direct interface for high-level, long-horizon reasoning. Prior work such as LLM-Planner~\cite{song2023llmplannerfewshotgroundedplanning} leverages visual inputs to decompose high-level plans into low-level actions, while CoELA~\cite{zhang2024buildingcooperativeembodiedagents} employs a rule-based executor only. In contrast, our design is more comprehensive: it supports both rule-based and LLM-based executors, processes inputs in both natural language and visual modalities, and is tightly coupled with our extendable simulator.

Our local action planner consists of two components: a \textbf{parser} and an \textbf{executor}. The parser receives high-level plans from an LLM and translates them into low-level executable actions. The executor then carries out these actions sequentially, conditioned on the environment state. To accommodate diverse research needs, we implement two executor variants: \textbf{rule-based} and \textbf{visual-based}. The rule-based executor operates on abstract city layout information, while the visual-based executor directly consumes visual inputs from the simulator, enabling seamless integration with VLMs.

For non-atomic actions such as navigation, the rule-based executor leverages a A* route planner to provide ground-truth paths, ensuring that natural language descriptions can be reliably mapped to executable sequences. Conversely, the visual-based executor passes raw visual observations to a backbone VLM, allowing the model to determine the next action, thereby testing its planning capabilities in complex environments.

For example, when local action planner receives a user plan such as ``go to the nearest chair and sit down,'' it decomposes the instruction into an action list: \textit{navigate}, \textit{agent\_sit\_down}. The \textit{navigate} action is not atomic but further decomposable into primitive actions such as \textit{step\_forward} and \textit{rotate}. In the rule-based mode, the planner first computes the shortest path from the agent's current position to the nearest chair, which results in a sequence of navigation primitives such as $navigate(0, 1)$, $navigate(1, 10)$, and $navigate(10, 10)$, where $(10, 10)$ is the chair’s location. Once the agent reaches the chair, the planner proceeds to $agent\_sit\_down$ and completes execution as the action list becomes empty. In contrast, the visual-based mode directly feeds environment observations to a VLM, which decides the next action step by step (e.g., $step\_forward$, $step\_forward$, $agent\_sit\_down$) relying on visual information.


\subsection{Task Suite Creation Workflow (New)}

To encourage widespread adoption, \simworld is built with extensibility and benchmark creation as core design goals. It provides tools to easily define tasks, agent roles, reward functions, and evaluation metrics—minimizing the engineering effort required to create new experiments. Figure~\ref{fig:workflow} showcases how to define a multi-agent delivery task within \simworld ecosystem. The process is delineated as follows:

First, users curate their own delivery datasets, either through the \simworld API or via custom pipelines (e.g., defining delivery locations, obstacles, and package types). Second, the delivery environment is instantiated on the \simworld UE side, incorporating realistic physical interactions such as traffic rules, dynamic pedestrians, and weather, along with high-fidelity visual perception. Third, LLM/VLM models are integrated as the decision-making core of the embodied delivery agent, enabling both route planning and interaction reasoning. Fourth, the benchmark information—datasets, environment configurations, and agent models—is hosted within the platform to ensure standardized experimentation. Finally, agents are ready for evaluation across multiple dimensions: efficiency (e.g., delivery success rate, average completion time), safety (e.g., number of collisions, traffic violations), and compliance (e.g., adherence to delivery constraints, respecting no-entry zones).



\newpage

==> sections/old-04-agent-interface.tex <==
\section{LLM/VLM Agents Interface}



==> sections/old-04-embodied-experiments.tex <==
\section{Embodied Experiments}

\subsection{Multi-modal Robot Navigation}

\subsubsection{Formulation}

\begin{figure}[!t]
    \centering
    % \vspace*{-60 pt}
    \includegraphics[trim=0cm 9.5cm 0cm 2.8cm, clip, width=\linewidth]{figures/section_5_single_agent.pdf}
    \vspace*{-20pt}
    \caption{Illustration of a multimodal robot navigation task.} 
    \vspace*{-20pt}
    \label{fig:embodied-single-agent-task} 
\end{figure}

Each navigation task consists of a series of multimodal instructions $I_{1\ldots K}$ that the robot must interpret and execute. As illustrated in Figure~\ref{fig:embodied-single-agent-task}, each instruction $I_k$ includes a natural language instruction and a visual hint illustrating what the robot can expect to see after reaching the goal described in the language instruction. These two modalities together guide the robot toward a specific location and/or orientation. Each instruction is associated with a ground-truth goal $g_k$. At any given timestep, only one instruction is presented to the robot, which must successfully complete the current instruction (i.e., reaching $g_k$) before receiving the next instruction $I_{k+1}$. 

To closely mirror real-world navigation challenges, the environments simulated incorporate both static obstacles (e.g., buildings, barriers) and dynamic agents (e.g., pedestrians, vehicles) whose trajectories are not known in advance. Task difficulty is determined by the complexity of the environment, and we define two levels: an \textit{easy} task includes no obstacles (static objects outside of buildings, pedestrians or vehicles), and a \textit{hard} task adds both static object obstacles and dynamic pedestrians and vehicles.

\subsubsection{Action Space}

The robot’s action space consists of two categories: movement actions and task-related actions. In the movement category, the robot can choose from the following options: move forward, move backward, move left, move right, turn left ($-90^\circ$), turn right ($+90^\circ$), or stay still. In the task-related category, the robot can select the action \texttt{evaluate}, indicating that it believes the current task has been completed. If the evaluation is correct, the robot receives the next subtask’s language instruction and visual hint; otherwise, the episode terminates as a failure.

\subsubsection{Observation Space}

Apart from the subtask description and expected visual hint, the robot has access to the egocentric RGB image, segmentation image, and depth image. Ground truth orientation is provided, assuming a built-in compass in the robot. 

\subsubsection{Procedural Task Generation}
\vspace{-9 pt}
\input{floating/algorithms/embodied_single_agent_task_generation}
As mentioned, we have two difficulty levels: \textit{easy} (without obstacles) and \textit{hard} (with obstacles such as vehicles and pedestrians). We generate 200 city maps using our procedural city generation pipeline in~\ref{algo1}, with 100 maps allocated to each setting. For the map under hard setting, streetside obstacles are additionally generated. 

On each generated map, we randomly sample a pair of points, denoted as $P_\text{start}$ and $P_\text{goal}$. For each point, we locate the nearest landmark building and extract the front-door location, referred to as $L_\text{start}$ and $L_\text{goal}$ respectively. The robot is spawned at $L_\text{start}$ and tasked with navigating to $L_\text{goal}$.

We then use the A* algorithm to compute an optimal path between $L_\text{start}$ and $L_\text{goal}$ over the city-wide waypoint graph.

This path is then decomposed into a sequence of subtasks (detailed in Algorithm~\ref{alg:mmnav-task-gen}):

\begin{itemize}
\item \textbf{Orientation Alignment:} The initial subtask, providing a target compass direction and a nearby landmark to assist robot alignment, accompanied by an initial visual cue.
\item \textbf{Move Along the Road:} Generated when the robot is expected to travel straight between two intersections, using a prominent landmark for navigation and capturing a visual cue at the next intersection.
\item \textbf{Turning at Intersections:} Inserted when a change in orientation is detected in the path (typically at an intersection), immediately following the previous move along the road step. It dictates a left or right turn based on the relative angle to the next waypoint and includes a new visual cue captured with the updated heading. 
\end{itemize} 
These \textbf{Move Along the Road} and \textbf{Turning at Intersections} subtasks may repeat multiple times until the robot reaches the final waypoint along the planned path.

\begin{itemize}
\item \textbf{Reach Destination:} The final subtask, providing a detailed description of the goal building and its spatial relationship to the robot's position, paired with a visual cue facing the destination.
\end{itemize}

This process completes one full navigation episode. For each map, we generate two navigation episodes by sampling different start and goal locations, resulting in a total of 400 navigation tasks (200 under the easy setting and 200 under the hard setting).

\subsubsection{Training Set Generation}

The training dataset is generated using a distinct set of maps, referred to as training maps, which differ from those used for evaluation. The primary difference lies in the building distribution: training maps include only 66\% of the building types that appear in the testing maps. The remaining 34\% of building types are held out exclusively for testing, ensuring a clear separation between seen and unseen environments and promoting better generalization.

We generated 100 training maps using only the selected 66\% of building assets. On each map, two tasks are sampled, resulting in 200 ground-truth trajectories. Each trajectory contains, on average, 100 steps, forming a training corpus of 20K steps.

At each step during training, the robot receives a synthesized observation and a corresponding sub-instruction, and is required to predict the correct next action. To enhance the robot's ability to reason about the goal and environment, we supervise not only the action prediction but also several intermediate reasoning targets. Specifically, the robot is trained to jointly predict: (1) the distance between the current observation and the target visual hint; (2) the orientation of the visual hint; and (3) the potential sequence of actions from the current location to the final goal. All of these supervisory signals are paired with ground-truth annotations and serve as multi-task learning objectives, guiding the robot toward a deeper understanding of spatial context and task intent.

\subsubsection{Metrics}

We evaluate Single-Agent Instruction Following using three metrics: Success Rate (SR), Subtask Success Rate (SSR), and Distance Progress (DP).

\paragraph{Success Rate} This metric measures the proportion of navigation tasks in which the agent successfully reaches the final destination. A trial is counted as successful only if the agent stops near the correct landmark building and is oriented towards it at the end of the trajectory.

\paragraph{Subtask Success Rate} This metric evaluates the proportion of correctly completed subtasks within a navigation episode. Let $N$ denote the total number of subtasks in a given instruction, and $n_c$ the number of subtasks successfully completed by the agent. The Subtask Success Rate (SSR) for that episode is computed as:
\begin{equation}
\text{SSR} = \frac{n_c}{N}
\label{eq:ssr}
\end{equation}
We report the average SSR across all test episodes.

\paragraph{Distance Progress} This metric quantifies how much closer the agent is to the goal at the end of the navigation compared to the beginning. Let $d_0$ be the initial distance to the goal and $d_T$ the final distance. The Distance Progress (DP) is computed as:
\begin{equation}
\text{DP} = \max\left(\frac{d_0 - d_T}{d_0}, 0\right)
\label{eq:dp}
\end{equation}
DP values are also averaged across all tasks to obtain the final score. All distances are computed using the Manhattan metric.

In the more challenging environment containing obstacles, pedestrians, and vehicles, we additionally measure three metrics to assess the robot's social navigation capabilities: the average number of static collisions (i.e., collisions with buildings or static obstacles), the average number of dynamic collisions (i.e., collisions with pedestrians or vehicles), and the number of actions that violate traffic light rules during navigation.

\subsubsection{Result}

Inspired by the recent success of large vision-language models (VLMs) on navigation tasks, we evaluate multiple recent VLMs as backbones for a common LLM-based planning framework, ReAct. We test GPT-4o , Gemini 2.5 Flash , Qwen-VL 2.5 7B, Qwen-VL 2.5 72B, Gemma 3 27B , InternVL2 2.5 8B and InternVL 3 78B. 

Each baseline equipped with a specific VLM backbone follows the same structured reasoning and action-planning process in ReAct. Additionally, we finetune QwenVL2.5-7B on our training set. Detail of the finetuning process can be found in Appendix. 

\input{tables/embodied_single_agent_easy}
\input{tables/embodied_single_agent_hard}

As shown in Table~\ref{tab:single-agent-benchmark}, among zero-shot ReAct models, Gemini 2.5 Flash achieves the highest progress score. GPT-4o exhibits a mismatch between its distance progress and subtask completion rate, primarily due to its inability to detect termination conditions, often overshooting the goal and yielding zero distance progress. QwenVL2.5-72B ranks highest among open-source models, while QwenVL2.5-7B performs comparably to significantly larger models. 

After fine-tuning, QwenVL2.5-7B shows substantial improvements across all metrics and is the only model to achieve a non-zero full task success rate. However, the absolute success rate remains low, partly because the training set is grounded on oracle action traces, which limits robustness. Incorporating reinforcement learning or corrective demonstrations could further enhance performance.

All zero-shot models score zero in full task success, highlighting a fundamental capability gap. Case studies suggest that these models often fail in task completion due to insufficient instruction grounding or inability to handle long-horizon dependencies.

We summarize typical failure modes as follows, with specific qualitative examples detailed in the supplementary material.

(1) \textbf{Visual Grounding.} The grounding of vision language model hinders its performance. The model fails to recognize the intersection, which is vital in our setting. The relatively low perspective of the robot dog add to the difficulties. (2) \textbf{Spatial and Embodied Reasoning.} VLMs do not yet have good 3D spatial reasoning capacity. It is still hard for robot to tell how close it is to a certain intersection or an obstacle. (3) \textbf{Pragmatic Thinking.} To emulate real-world textual navigation, our instructions use high-level phrases like "turn right at the intersection" without detailing the specific turning and crossing actions required. Most models fail to interpret such ambiguity correctly. (4) \textbf{Memory and Planning.} VLMs sometimes fail to adapt the information in memory to the current situation.

\subsection{Multi-robot Search}

\subsubsection{Formulation}

\begin{figure}[!t]
    \centering
    % \vspace*{-60 pt}
    \includegraphics[trim=0cm 8.5cm 0cm 2.8cm, clip, width=\linewidth]{figures/section_5_multi_agents.pdf}
    \vspace*{-20pt}
    \caption{Illustration of a multi-robot search task.} 
    \vspace*{-20pt}
    \label{fig:embodied-multi-agent-task} 
\end{figure}

As illustrated in \ref{fig:embodied-multi-agent-task}, there are two robots, a main robot and a follower robot spawned in different locations at the same city environment. The main robot has explored the city, so it has the memory of a map and images of landmarks (typically over 20 landmarks) in the city. However, the follower robot is new to the city and does not have such information. Neither robot knows the other's location. Their goal is to meet each other as soon as possible by physical navigation as well as verbal communication. A task is considered successful when at least one of the robots confirms that it can see the other robot in its egocentric view.

\subsubsection{Action Space}

Besides the actions available in the multi-modal robot navigation task, the robot can additionally choose to send natural language messages to other agents. All other movement (forward, backward, left, right, turn $\pm90^\circ$, stay still) and task-related (evaluate) actions remain the same.

\subsubsection{Observation Space}

In addition to all the observation space in the multi-modal robot navigation task, the robot can also observe natural language messages sent by other agents.

\subsubsection{Task Generation}

To construct the tasks for multi-robot search, we procedurally generate 100 unique city maps using procedural city generation pipeline in~\ref{algo1}, each covering a large-scale urban environment. For each map, we instantiate one multi-robot search task, resulting in a total of 100 evaluation tasks. The task generation process follows Algorithm~\ref{alg:mrs-task-gen}.

\input{floating/algorithms/embodied_multi_agent_task_generation} 

Specifically, we first sample $n$ landmark buildings along each of the $m$ streets in the city and collect their front-door images with aligned orientations. These image-location pairs serve as the main robot's memory of the city. Next, we sample two distinct and valid spawn locations as the starting positions for the main robot and the following robot. This ensures spatial diversity and supports realistic localization and communication challenges.

\subsubsection{Metrics}

We report two metrics for evaluating performance on the Multi-Robot Search task: Collaborative Success Rate (CSR) and Task Progress (TP).

\paragraph{Collaborative Success Rate}  
This metric estimates the probability that the two robots successfully meet up across different maps. A meet-up is considered successful if at least one robot executes the \texttt{evaluate} action and detects the other robot dog in its observation via ground-truth segmentation. 

\paragraph{Task Progress}  
This metric quantifies the relative reduction in distance between the two robots by the end of the task. Let $D_0$ denote the initial distance between the two agents, and $D_T$ the distance when the task terminates. The Task Progress (TP) is defined as:
\begin{equation}
\text{TP} = \max\left(\frac{D_0 - D_T}{D_0}, 0\right)
\label{eq:task_progress}
\end{equation}

\subsubsection{Results}
\input{tables/embodied_multi_agent}

Table~\ref{tab:multi-benchmarks} summarizes baseline results on our multi-robot search task. GPT-4o with the oracle planner achieves the highest CSR (52\%) and task progress (68.44\%) by combining precise landmark localization with optimal A* planning, showing upper-bound performance with full map access. The RoCo policy lets the follower describe its view, which the map-aware robot localizes via VLM-based retrieval. This one-shot communication enables concurrent movement and more realistic coordination. However, converting rendezvous plans into language introduces ambiguity and execution noise, often causing path deviations. Without iterative replanning, grounding or control errors can't be corrected. Consequently, GPT-4o under RoCo achieves only 33.33\% CSR and 22.93\% task progress—significantly lower than the oracle baseline.

==> sections/old-05-agent-experiments.tex <==
\section{Agent Experiments}
\subsection{Agent Physical Reasoning Experiment}
\subsubsection{Formulation}
To evaluate the embodied reasoning and physical interaction capabilities of agents within \simworld, we introduce a vision-based navigation task in urban environments. Agents are tasked with reaching a specified destination while avoiding both static obstacles (e.g., trees, benches) and dynamic agents (e.g., pedestrians), necessitating strong spatial reasoning and multimodal perception under uncertainty. The task requires agents to process real-time visual input and make sequential decisions to avoid collisions, respect traffic rules, and reach the goal efficiently.

To analyze the interplay between high-level planning and low-level reactive control, we consider two settings: \textit{with} and \textit{without} a Local Action Planner. In the Local Action Planner setting, agents are guided by a precomputed global route generated via A* search, which omits obstacle information. Agents must navigate from one waypoint to the next along this route while handling local interactions. In the planner-free setting, agents receive only the goal position and are expected to autonomously plan and execute a safe trajectory.

\subsubsection{Action Space}
Each agent may choose from the following actions at each decision step:
\begin{itemize}[noitemsep,leftmargin=10pt]
    \item \textbf{Do Nothing}: Remain stationary.
    \item \textbf{Step}: Move forward or backward for a fixed duration.
    \item \textbf{Turn}: Rotate left or right by any angle (continuous range).
    \item \textbf{Change Next Waypoint}: (Local Action Planner only) Switch to a different candidate waypoint.
\end{itemize}

\subsubsection{City Map and Task Generation}
\begin{itemize}[noitemsep,leftmargin=10pt]
    \item \textbf{Coarse-grained Map}: Each sidewalk is divided into three waypoints (start, midpoint, end), forming a navigation graph to generate tasks.
    \item \textbf{Fine-grained Map}: Each sidewalk is sampled with $\sim$70 evenly spaced waypoints. These serve both as candidate motion targets and obstacle anchor points.
    \item \textbf{Obstacles}: Static objects (trees, trash bins, etc.) are randomly placed on fine-grained waypoints. Dynamic pedestrians follow sidewalk paths at moderate speed with randomized starting positions.
\end{itemize}

Figure~\ref{fig:expr1-task-generation} illustrates the task generation pipeline. We begin with a basic road network provided by SimWorld, which includes sidewalks, crosswalks, and intersection nodes. To construct the coarse-grained navigation graph, we interpolate a midpoint for each sidewalk segment, yielding a simplified map structure suitable for high-level planning.

Tasks are generated by randomly sampling start and goal nodes from this graph, with constraints on the number of segments between them to control difficulty. For fine-grained navigation, we densify the original sidewalk geometry by interpolating evenly spaced waypoints. Each sidewalk is divided into four lateral lanes, each containing 17 waypoints, while each crosswalk contains 8 waypoints.

To simulate realistic urban clutter, we place static obstacles such as trees and street furniture along these waypoints. Trees are sampled on the innermost lane (nearest to buildings) of each sidewalk, while other street elements (e.g., benches, trash bins) are distributed across the remaining three lanes. Importantly, for each group of four laterally aligned waypoints (i.e., across the four sidewalk lanes at the same longitudinal position), at least one is guaranteed to remain obstacle-free. This ensures that there is always a traversable option at every step along the sidewalk.

We sample 40 tasks spanning the four difficulty levels:
\begin{itemize}[noitemsep,leftmargin=10pt]
    \item Easy (10 tasks), Medium (10 tasks), Hard (10 tasks), Dynamic (10 tasks).
    \item Each task is defined by a sequence of waypoints $T_i = [W_1, W_2, ..., W_n]$.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Exp1-task.pdf}
    \caption{\textbf{Task Generation Pipeline for Physical Reasoning Experiment.}}
    \label{fig:expr1-task-generation}
\end{figure}

\subsubsection{Baseline Agent Protocols}
\begin{itemize}[noitemsep,leftmargin=10pt]
    \item \textbf{Rule-based Agent}: Follows Local Action Planner waypoints using a fixed stepping strategy. Obey the traffic rules and does not observe visual input or adapt to obstacles.
    \item \textbf{VLM Agents}:
    \begin{itemize}
        \item Input: current image, last-step image, past 3 actions and feedback, current navigation goal, relative distance and angle to current navigation goal.
        \item Output: action selected from the predefined space.
        \item Perception is simulated via RGB screenshots with 90° horizontal FOV.
    \end{itemize}
\end{itemize}

\subsubsection{Metrics}
Throughout the experiment, we evaluate agent performance using the following six metrics, which together capture task success, safety compliance, and decision efficiency:

\begin{itemize}[noitemsep,leftmargin=10pt]
    \item \textbf{Success Rate (SR)}: The percentage of navigation tasks in which the agent successfully reaches its destination without getting stuck, timing out, or deviating significantly from the designated route. This metric reflects the overall effectiveness of the agent's decision-making and path-following capabilities. 
    \[
    \text{SR} = \frac{N_{\text{success}}}{N_{\text{total}}}
    \]
    
    where \(N_{\text{success}}\) is the number of successfully completed tasks, and \(N_{\text{total}}\) is the total number of tasks.
    
    \item \textbf{Collision Count (CC)}: The total number of collisions that occur between the agent and either static obstacles (e.g., trees, trash bins) or dynamic entities (e.g., pedestrians). A lower collision count indicates better obstacle avoidance and situational awareness. Collisions are recorded for all episodes, regardless of success or failure.

    \[
    \text{CC} = \sum_{i=1}^{N_{\text{total}}} c_i
    \]
    
    where \(c_i\) is the number of collisions in episode \(i\).
    
    \item \textbf{Collision Count (Success Only) (CC-S)}: The number of collisions occurring only within successful episodes, which reflects if the agent really avoids the obstacles. Since the CC is possibly low if the agent get stuck at the very beginning. This metric helps assess how safely the agent completes tasks when it does reach the goal.
    \[
    \text{CC-S} = \sum_{i \in \mathcal{S}} c_i
    \]
    
    where \(\mathcal{S}\) is the set of successful episode indices.
    
    \item \textbf{Red-light Violation Rate (RVR)}: The fraction of successful episodes in which the agent crosses an intersection during a red traffic signal, violating traffic rules. This metric evaluates the agent’s ability to obey traffic signals and is computed only over successful episodes to ensure fair assessment under comparable task completion.

    \[
    \text{RVR} = \frac{\sum_{i \in \mathcal{S}} r_i}{|\mathcal{S}|}
    \]
    
    where \(r_i = 1\) if a red-light violation occurred in episode \(i\) and 0 otherwise, and \(|S|\) is the total number of successful episodes.
    
    \item \textbf{Stuck Rate (STR)}: The percentage of failed episodes in which the agent remains unable to reach the destination due to either physical immobilization (e.g., blocked by obstacles) or ineffective decision-making (e.g., repeatedly turning or repositioning without forward movement) over a period of 2 minutes. STR captures both hard failures (being physically stuck) and soft failures (behavioral indecision), reflecting challenges in planning and low-level control.

    \[
    \text{STR} = \frac{N_{\text{stuck}}}{N_{\text{failed}}}
    \]
    
    where \(N_{\text{failed}} = N_{\text{total}} - N_{\text{success}}\) and \(N_{\text{stuck}}\) is the number of failed episodes classified as stuck.
    
    \item \textbf{Normalized Decision Count (NDC)}: The ratio between the total number of decision-making by the large model and the total number of fine-grained waypoints provided by the Local Action Planner, computed over successful episodes. NDC measures the agent’s decision efficiency, with a lower value indicating more economical use of the model.

    \[
    \text{NDC} = \frac{1}{|\mathcal{S}|} \sum_{i \in \mathcal{S}} \frac{d_i}{w_i}
    \]
    
    where \(d_i\) is the number of model decisions made in episode \(i\), and \(w_i\) is the number of fine-grained waypoints along the successful path. \(|S|\) is the total number of successful episodes.

    \item \textbf{Decision Steps in Success (DSS)}: The average number of decision-making steps taken by the large model in episodes that were successfully completed. DSS measures the typical number of decisions required to achieve a successful outcome, with a lower value potentially indicating more efficient or direct decision-making in successful scenarios.
    
    \[
    \text{DSS} = \frac{1}{|\mathcal{S}|} \sum_{i \in \mathcal{S}} d_i
    \]
    
    where \(d_i\) is the number of model decisions made in successful episode \(i\), and \(|S|\) is the total number of successful episodes.
\end{itemize}

Together, these metrics provide a comprehensive evaluation of an agent’s navigation performance, safety behavior, and decision-making efficiency in complex urban environments.

\subsubsection{Main Results: Agent Planning With Local Action Planner}
\paragraph{Static Obstacle.} 
We evaluate three levels of task difficulty (Easy, Medium, Hard) under static obstacles with a local action planner. Time limits are set to 15 minutes for Easy and Medium tasks, and 25 minutes for Hard tasks. Four VLMs are evaluated: GPT-4o-mini, \texttt{GPT-4o}, \texttt{Claude-3.7-Sonnet}, and \texttt{Gemini-2.5-Pro} (gemini-2.5-pro-preview-03-26). Results are shown in Table~\ref{tab:baseline-difficulty}, with key insights discussed below:

\input{tables/physical_baselines}

\textit{Model capability is a decisive factor in task success.} State-of-the-art models such as \texttt{GPT-4o}, \texttt{Claude-3.7-Sonnet}, and \texttt{Gemini-2.5-Pro} consistently outperform the rule-based baseline across all three difficulty levels. These advanced VLMs achieve higher SR, along with lower CC and CC-S, indicating their ability to understand the environment and avoid obstacles more effectively. In contrast, \texttt{GPT-4o-mini} performs even worse than the rule-based baseline, with lower SR and higher CC and CC-S, suggesting that it struggles to follow task rules and may be prone to hallucinations or unreasonable actions.

\textit{VLMs demonstrate limited spatial reasoning.} Although larger VLMs attain higher SR across all tasks, we do not observe a corresponding drop in CC or CC-S. This implies that while these models attempt to avoid obstacles, they often fail—frequently grazing or barely touching the edges of objects. This behavior suggests that current VLMs possess strong visual recognition abilities but lack a robust understanding of spatial relationships and depth.

\textit{Different models exhibit distinct strengths.} Our analysis reveals that individual models have specialized advantages. For instance, \texttt{GPT-4o} and \texttt{Claude-3.7-Sonnet} show higher STR, indicating that its failures are more often due to getting stuck rather than poor decisions, suggesting better decision-making but weaker spatial adaptability. In contrast, \texttt{Gemini-2.5-Pro} shows a lower STR, implying that it struggles more with planning and timely decision-making. These trends are consistent with their respective SR, CC, and CC-S values: \texttt{GPT-4o} and \texttt{Claude-3.7-Sonnet} excel in making quick and precise decisions, while \texttt{Gemini-2.5-Pro} shows better spatial comprehension. Figure \ref{fig:llm_choice_proportion} shows that \texttt{Gemini-2.5-Pro} performs "choose a new waypoint" more than other models, which further explains that \texttt{Gemini-2.5-Pro} are more sensitive to obstacle avoidance. Additionally, lower NDC supports these findings by showing which models complete tasks using fewer steps, reflecting planning efficiency.

\textit{VLMs fail to function as truly embodied agents.} Although VLM-driven agents do not achieve 100\% RVR in the table, additional experiments on the Hard tasks—where all pedestrian signals were kept red—reveal a more fundamental issue: agents crossed streets despite the red lights. To correctly perceive the signal state, an agent must look up and focus on the signal. Upon detecting a red light, it should repeatedly choose the \textit{do nothing} action until the signal turns green. However, experimental results show that none of the agents chose to adjust their view, and very few opted to do nothing, indicating that VLMs do not recognize their ability to adjust visual sensors. Instead, they react only based on the input they are given. This suggests that LLM-based agents require substantial additional components to behave like real embodied agents—the LLM alone is not sufficient.


\begin{AIbox}{Takeaway: Replanning with Static Obstacles}
Model capability plays a decisive role in determining task success, yet current VLMs exhibit limited spatial reasoning and consistently fall short of functioning as truly embodied agents. Despite this, different models display distinct operational strengths, indicating varied but incomplete competencies across the board.
\end{AIbox}

\input{floating/images/physical_choice_proportion}

\paragraph{Dynamic Obstacles.} 
Table \ref{tab:baseline-dynamic} presents the performance of different models on dynamic navigation tasks. \texttt{GPT-4o} and \texttt{Claude-3.7-Sonnet} demonstrate superior performance, achieving higher SR and lower NDC. This suggests that these models are capable of making faster and more decisive actions, enabling them to complete navigation tasks efficiently in dynamic environments. In contrast, \texttt{Gemini-2.5-Pro} experiences a significant drop in SR and exhibits higher NDC values—comparable to those of \texttt{GPT-4o-mini}—while also recording the lowest values in both CC and CC-S among all baselines.

Figure~\ref{fig:llm_choice_proportion} reveals that \texttt{Gemini-2.5-Pro} frequently switches waypoints and tends to choose valid ones, suggesting stronger spatial sensitivity. However, this caution often leads to hesitation or stalls near moving obstacles, highlighting a trade-off between spatial adaptability and robust task completion.

\begin{AIbox}{Takeaway: Replanning with Dynamic Obstacles}
\texttt{GPT-4o} and \texttt{Claude-3.7-Sonnet} excel in dynamic scenarios with high task success and efficient decision-making. \texttt{Gemini-2.5-Pro} shows superior obstacle sensitivity, achieving the fewest collisions, but its cautious behavior leads to more frequent stalls and lower task success (Table~\ref{tab:baseline-dynamic}).
\end{AIbox}

\input{tables/physical_dynamic}
\input{tables/physical_ablation}

\subsubsection{Ablation Study: Without Local Action Planner}
To evaluate the robustness of VLM-driven agents under more challenging conditions, we remove the local action planner and re-evaluate their performance on Medium-level tasks. In this setting, agents are only provided with the final destination instead of a pre-defined series of waypoints. They are required to not only avoid collisions but also plan an efficient trajectory autonomously. All agents are restricted to a maximum of 90 decision steps per task.

We compare three state-of-the-art VLMs: \texttt{GPT-4o}, \texttt{Claude-3.7-Sonnet}, and \texttt{Gemini-2.5-Pro} (gemini-2.5-pro-preview-05-06). As shown in Table \ref{tab:baseline-non-planner}, \texttt{GPT-4o} fails to complete any task successfully (SR = 0), while \texttt{Claude-3.7-Sonnet} achieves a 56.67\% SR and it also achieves the lowest DSS of 58.71, indicating more efficient decision-making. \texttt{Gemini-2.5-Pro} outperforms both with the highest SR (60.0\%) and the lowest overall CC (16.23), including significantly fewer building and object collisions.

\input{floating/images/physical_distance}

Figure \ref{fig:combined-distance} illustrates the distance-to-goal progression for each model from a single experimental run. The behavioral patterns underlying these distance trends are further elucidated by Figure \ref{fig:llm_choice_proportion}, which shows \texttt{GPT-4o} and \texttt{Claude-3.7-Sonnet} frequently engaging in non-progressive turning actions, whereas \texttt{Gemini-2.5-Pro} predominantly maintain forward movement.



\begin{AIbox}{Takeaway: Navigation without Local Action Planner}
\texttt{Gemini-2.5-Pro} demonstrates superior autonomous planning and obstacle avoidance without local guidance, while \texttt{Claude-3.7-Sonnet} is efficient but less safe. \texttt{GPT-4o} fails to adapt without pre-defined waypoints (Table~\ref{tab:baseline-non-planner}).
\end{AIbox}

\subsubsection{Prompt Design}
\begin{promptbox}{System Prompt of Navigation Task with Local Action Planner}
\lstinputlisting[language=Octave,style=mystyle]{prompts/vlm_system_prompt.py}
\end{promptbox}
\label{tab:exp1_sys_prompts}

\begin{promptbox}{User Prompt of Navigation Task with Local Action Planner}
\lstinputlisting[language=Octave,style=mystyle]{prompts/vlm_user_prompt.py}
\end{promptbox}
\label{tab:exp1_user_prompts}

\begin{promptbox}{System Prompt of Navigation Task without Local Action Planner}
\lstinputlisting[language=Octave,style=mystyle]{prompts/vlm_system_prompt_without_planner.py}
\end{promptbox}
\label{tab:exp2_sys_prompts_non_planner}

\begin{promptbox}{User Prompt of Navigation Task without Local Action Planner}
\lstinputlisting[language=Octave,style=mystyle]{prompts/vlm_user_prompt_without_planner.py}
\end{promptbox}
\label{tab:exp2_sys_prompts_non_planner}

\subsubsection{Chain of Thought Example}
This section, we showcase a representative chain of thought from \texttt{Gemini-2.5-Pro} as it navigated the Easy level task. This demonstration is provided to give readers a transparent view of the model's deliberative process when prompted to "think step-by-step." The following transcript captures the VLM's sequential reasoning, from understanding the prompt to formulating its next action.
\begin{promptbox}{Example Chain of Thought from \texttt{Gemini-2.5-Pro} on a Successful Easy Task}
\lstinputlisting[language=Octave,style=mystyle]{prompts/reasoning.py}
\end{promptbox}
\label{tab:exp2_sys_prompts_non_planner}


\subsection{Agent Social Reasoning Experiment}
In this section, we deploy a strategic multi-agent collaboration and competition task designed to evaluate the performance of foundation model agents in realistic, open-world urban environments. Specifically, we simulate a delivery platform as the context of this setting for case study. 

\boldstart{Formulation.}
To evaluate the social reasoning capabilities of foundation models in realistic, open-world urban environments, we propose a strategic multi-agent delivery task that involves both collaboration and competition.
LLM-based agents are deployed as delivery personnel in a city-scale environment built using \simworld. Their goal is to grow and thrive in this dynamic setting. To enhance realism and complexity, the environment incorporates several dynamic systems:
(1) an energy system, where agents must manage stamina and replenish it through consumables;
(2) an economic system, where agents earn and spend currency on purchases such as scooters and drinks;
(3) an order-sharing mechanism, enabling agents to collaborate by sharing delivery tasks and optimizing group performance.
These components create a rich, interactive simulation environment for evaluating agents’ decision-making, adaptability, and social reasoning in complex urban scenarios.

Let the set of \textit{Delivery Agent} be represented as \( \mathcal{D} = \{D\_1, D\_2, \dots, D\_n\} \), each operating independently yet concurrently in the shared environment.

At each discrete timestep \( t \), an agent \( D\_i \) chooses from the following set of actions:
\begin{enumerate}[noitemsep,leftmargin=10pt]
    \item Accept or reject available orders.
    \item Plan routing along waypoints defined by a provided map structure.
    \item Purchase transportation equipment to enhance delivery efficiency, subject to available financial resources.
    \item Adjust travel speed \( v\_t \in [v\_{\text{min}}, v\_{\text{max}}] \) to balance energy consumption and delivery speed.
\end{enumerate}

Each \textit{Delivery Agent} \(D\_i\) operates under the following constraints:

\begin{itemize}[noitemsep,leftmargin=10pt]
    \item \textbf{Energy Constraint}: Agent \( D\_i \) has an energy level \(E\_t \geq 0\). Movement at higher speeds consumes more energy, and energy can be replenished by purchasing beverages at supply points.
    \item \textbf{Financial Constraint}: Each agent starts with an initial amount of money \(M\_0\). Actions such as purchasing transportation equipment or beverages require spending money. The agent's financial status at time \(t\) is represented by \(M\_t\geq 0\).
    \item \textbf{Spatial Constraint}: Movements must follow a predetermined waypoint map \(\mathcal{G} = (\mathcal{V}, \mathcal{E})\), where \(\mathcal{V}\) is the set of waypoints, and \(\mathcal{E}\) represents feasible paths.
\end{itemize}

The primary objective for each \textit{Delivery Agent} \(D\_i\) is to maximize total money \(M\_T\) accumulated by the end of simulation period \(T\):

\begin{equation}
    \max \quad M\_T = M\_0 + \sum\_{t=1}^{T} (R\_t - C\_t)
\end{equation}

where \(R\_t\) represents revenue earned at timestep \(t\) from successful deliveries. \(C\_t\) represents costs incurred at timestep \(t\), including equipment purchase costs, energy replenishment costs, and penalties from delayed or failed deliveries.

Agent dynamics at timestep \(t\) are governed by:
\begin{align}
    E\_{t+1} &= E\_t - f(v\_t) + \Delta E\_{\text{replenish}},\\
    M\_{t+1} &= M\_t + R\_t - C\_t,\\
    X\_{t+1} &= \text{WaypointUpdate}(X\_t, a\_t),
\end{align}

where: \(f(v\_t)\) denotes energy consumption as a function of travel speed. \(\Delta E\_{\text{replenish}}\) is the energy replenished through beverages at supply points. \(X\_t\) denotes the agent's position at timestep \(t\), updated based on actions \(a\_t\) following the waypoint system.

This formulation offers a comprehensive framework for evaluating long-horizon decision-making strategies of \textit{Delivery Agents} within the multi-agent environment of \simworld.

\boldstart{Environment.}
All experiments are conducted on the same map generated by \simworld. To ensure fair and efficient evaluation, graphical rendering is disabled during simulation. However, the physical simulation and evaluation threads remain active to preserve environment dynamics and task fidelity.

\boldstart{Action Space.}
The task features a two-tiered action space: high-level actions decided by LLM agents and low-level actions executed by the \simworld local action planner. At each decision step, the agent may choose: \textbf{Bid Order} (offer a price to compete for a new order), \textbf{Pick Up Order} (navigate to the pick-up point), \textbf{Deliver Order} (complete delivery at the destination), \textbf{Share Order} (publish the order for collaboration), \textbf{Cancel Share Order} (withdraw a previously shared order), \textbf{Go to Meet-point} (head to the coordination point for a shared order), \textbf{Purchase Drinks} (buy consumables to restore energy), or \textbf{Adjust Speed} (cancel order or modify travel speed dynamically). Full action space is shown in Table \ref{tab:delivery-action-space}.
\input{floating/tables/delivery_actionspace}

\boldstart{Baseline Agents.}
We evaluate multiple foundation models as the backbone of delivery agents, including \texttt{Claude-3.5-Sonnet}, \texttt{DeepSeek-V3}, \texttt{GPT-4o}, \texttt{Gemini-2.5-Flash}, and \texttt{QWQ}. The ReAct~\cite{yao2023reactsynergizingreasoningacting} prompting framework is employed to explicitly separate reasoning and action selection. 
% Further implementation details can be found in Appendix~\ref{apdx:expr2}.

Multi-agent collaboration and competition settings has a two-layer hierarchical action space, which aligns closely with the local planner module for modular action execution. Specifically, the high-level decisions guide the agent's strategic behavior in the environment and the low-level actions are executed by local planner to update physical states. 
% The details of action space of strategic multi-agent collaboration and competition task is described in Appendix~\ref{apdx:exp2-actionspace}
% \input{tables/delivery_actionspace}



\begin{table}[ht]
\centering
\small
\vspace{-1em}
\setlength\tabcolsep{4.5pt}
\setlength\extrarowheight{2pt}
\caption{\textbf{Hierarchical action space of strategic multi-agent collaboration and competition task.} The high-level actions are generated by LLMs, the low-level actions are executed by local planner.}
% \vspace{-8pt}
\label{tab:deliverybench_action_space_compact}
\resizebox{\linewidth}{!}{
\begin{tabular}{l l l l}
\hline
\multicolumn{1}{c}{\bf \cellcolor[HTML]{D9EAD3} High-Level Actions} 
& \multicolumn{1}{c}{\bf \cellcolor[HTML]{FCE5CD} Low-Level Actions} \\
Bid Order, Pick Up Order, Deliver Order, Navigate to Point, Share Order,Purchase Scooter, 
& Move Forward \\
Cancel Share Order, Go to Meet-point, Purchase Drinks, Adjust Speed
& Rotate, Change Speed \\
\hline
\end{tabular}
}
\end{table}

Furthermore, multi-agent collaboration and competition settings integrates multiple dynamic systems to enhance the realism and complexity of the environment. These include an energy system, where agents must manage their stamina and replenish it through consumables; an economic system, where agents earn and spend currency on transactions such as purchasing scooters or drinks; and an order-sharing mechanism, which enables agents to cooperate by sharing tasks and optimizing collective performance. These integrated systems provide a rich and interactive simulation environment for evaluating agents' multi-faceted decision-making and cooperative behaviors.

\boldstart{Delivery Personas Hub.} Inspired by~\cite{ge2024scalingsyntheticdatacreation}, we developed a workflow to generate delivery‑scenario personas. For each agent, we assign diverse backgrounds, distinct Big Five personality profiles, varied physical abilities, and initial economic statuses. We then employ a large language model to integrate these attributes into cohesive persona descriptions that guide agent behavior across different scenarios. In our experiments, we selected ten representative personas and paired each with twelve mainstream language models, yielding 120 agents with varied backend configurations.

\boldstart{Metrics.} 
Aligned with the agent’s hierarchical decision-making, we design a three-level evaluation framework. Overall performance is measured by \textbf{total profit}, while \textbf{order success rate}, \textbf{energy efficiency}, \textbf{order sharing count}, and \textbf{investment count} assess operational effectiveness. Additionally, we validate individual actions against simulation rules to ensure stability and evaluate the agent’s instruction-following and rule compliance under complex constraints.

Aligned with our hierarchical evaluation framework, we define the following metrics for each agent \(D_i\) operating over \(T\) timesteps. For high‐level, we take the total profit as metric:
\begin{equation}
      P_i \;=\; M_i(T) \;-\; M_i(0)\,
\end{equation}
where \(M_i(t)\) is the agent’s monetary balance at time \(t\). And for low‐level we mainly consider the operational effectiveness from the following aspects:
\begin{align}
  \text{Order Success Rate:}\quad 
    \mathrm{SR}_i &= \frac{|\mathcal{O}_i^{\mathrm{succ}}|}{|\mathcal{O}_i^{\mathrm{bid}}|}\,, \\[4pt]
  \text{Delay Rate:}\quad 
    \mathrm{DR}_i &= \frac{|\mathcal{O}_i^{\mathrm{delay}}|}{|\mathcal{O}_i^{\mathrm{succ}}|}\,, \\[4pt]
  \text{Energy Efficiency:}\quad 
    \mathrm{EE}_i &= \frac{P_i}{\sum_{t=1}^T e_i(t)}\,, \\[4pt]
  \text{Order‐Sharing Number:}\quad 
    \mathrm{SH}_i &= |\mathcal{O}_i^{\mathrm{shared\_succ}}|,, \\[4pt]
   \text{Investment Number:}\quad
    \mathrm{IN}_i &= |\mathcal{A}_i^{\mathrm{buy\_bike\_succ}}| ,,
\end{align}
where \(\mathcal{O}_i^{\mathrm{bid}}\) is the set of orders on which \(D_i\) bid, \(\mathcal{O}_i^{\mathrm{succ}}\subseteq \mathcal{O}_i^{\mathrm{bid}}\) are those bids that led to successful deliveries, \(e_i(t)\) is energy consumed by \(D_i\) at timestep \(t\), \(\mathcal{O}_i^{\mathrm{delay}}\subseteq \mathcal{O}_i^{\mathrm{succ}}\) are deliveries completed after the deadline, \(\mathcal{O}_i^{\mathrm{shared\_succ}}\) denotes successfully shared orders. \(\mathcal{A}_i^{\mathrm{buy\_bike\_succ}}\) demotes successfully buy bike actions. These statistics are written to our CSV outputs for each model grouping. And we show the part of metric in the Table~\ref{tab:main_results}.



% More details in Appendix~\ref{apdx:expr2}.

\subsubsection{Main Results}
\label{sec4.2}
We utilize the OpenRouter\footnote{\url{https://openrouter.ai/}} APIs to access and query a variety of large language models. To ensure fair and efficient evaluation, we disable graphical rendering during simulation while retaining the physical simulation and evaluation threads to preserve environment dynamics and task realism. 

For each evaluation run, we sample 20 agents controlled by the same language model, each performing 5000 simulation steps. 
Our prompt design consists of three parts: A \emph{system prompt} containing the static, structured map data, which is cached to minimize token usage; A \emph{context prompt} encoding the current global state and per‐agent state information. To avoid prompt bloat when many orders are available, we restrict the number of visible orders to at most ten; A \emph{user prompt} containing the context prompt, and give the guidance of different structured formats output during reasoning stage and action stage.
We employ the ReAct~\cite{yao2023reactsynergizingreasoningacting} prompting framework to enforce an explicit reasoning step before action selection, which improves overall performance. 
At each timestep, an agent issues two API requests, consuming on average approximately 7000 tokens each request.
Following the performance evaluation detailed in Table~\ref{tab:main_results}, an empirical analysis across three simulation rounds highlights divergent operational profiles among the assessed models. 

Agents are evaluated along several key dimensions, including task execution, long-horizon planning, cooperation, and investment decision-making. These abilities are quantitatively measured using the following five metrics: \textit{Profit}, \textit{Success Rate}, \textit{Energy Efficiency}, and \textit{Sharing Rate}. The results are summarized in Table~\ref{tab:main_results}, offering a structured comparison of agent behaviors across different models and configurations.

\input{floating/tables/agent_experiment2_main}
In each evaluation, we sample 20 agents controlled by the same language model, each running for 5000 simulation steps. At every step, an agent issues two API requests, averaging approximately 7000 tokens per request. Based on results from three simulation rounds (see Table \ref{tab:main_results}), we conducted an empirical analysis of model behaviors under this setup.

The results reveal clear differences in performance across models in terms of profit, order completion, and energy efficiency. Models with higher average performance often exhibit greater variability, while more stable models tend to have moderate outcomes. Some models show extreme fluctuations in specific metrics, indicating unpredictable behavior. A few models consistently returned zero across all metrics, suggesting a failure to understand the task or act meaningfully. Overall, the findings highlight a key trade-off between optimizing for high average performance and ensuring stable, predictable behavior—an important consideration for deployment in dynamic environments.

For each evaluation, we sample 20 agents controlled by the same language model, each running for 5000 simulation steps. At each step, an agent issues two API requests, averaging around 7000 tokens per request. Based on results in Table \ref{tab:main_results}, empirical analysis over three simulation rounds reveals distinct operational behaviors across models.

% Key insights are discussed in Appendix~\ref{app:case2-main} and summarized below. 

\texttt{DeepSeek-V3} ($69.475 \pm 16.772$) and \texttt{Claude-3.5-Sonnet} ($69.068 \pm 20.685$) achieved the highest mean profits, with \texttt{Claude-3.5-Sonnet} also leading in mean successful orders ($2.733 \pm 1.102$) and energy efficiency ($0.5411 \pm 0.1981$). 
Notably, these superior average outcomes were associated with substantial performance variability, as reflected in their respective standard deviations. 

Conversely, \texttt{Gemini-2.5-Flash}, while attaining a moderate mean profit of $42.423$, exhibited markedly more consistent profit generation with a standard deviation of $\pm 3.103$, and also demonstrated stability in successful orders ($2.100 \pm 0.173$). 
Extreme variability was evident in specific metrics for certain models; for instance, sharing counts for \texttt{Deepseek-Prover-V2} ($7.333 \pm 8.386$) and \texttt{Claude-3.5-Sonnet} ($11.333 \pm 8.386$) showed standard deviations exceeding their means, indicating highly unpredictable behavior in this aspect. 

The \texttt{GPT-4o-mini} model consistently yielded zero values across all metrics ($0.000 \pm 0.000$), suggesting it does not truly understand the goals to make reasonable decisions based on the given instructions and context information. 

Higher investment strategies, such as those adopted by \texttt{DeepSeek-V3} ($8.000 \pm 3.000$) and \texttt{Claude-3.5-Sonnet} ($9.000 \pm 3.464$), generally correlated with greater mean profit achievement but also with increased outcome volatility. 
These findings underscore a prevalent trade-off between optimizing for peak average performance metrics and ensuring consistent, predictable agent behavior, a critical consideration for robust deployment in dynamic environments.

\begin{AIbox}{Takeaway: Model Performances in Multi-agent Tasks}
Top-performing models like \texttt{DeepSeek-V3} and \texttt{Claude-3.5-Sonnet} achieved high average profits but exhibited significant variability, while \texttt{Gemini-2.5-Flash} showed more stable, though moderate, performance. \texttt{GPT-4o-mini} failed entirely across all metrics. Overall, the results highlight a trade-off between maximizing average performance and ensuring consistent, reliable behavior.
\end{AIbox}

\subsubsection{Ablation Study} 
\label{sec4.3}
To take a step deeper on multi-agent collaboration and competition, we conduct three ablation experiments. \textbf{Model Competition}, we sample 24 agents and 12 models that each model control two agents running experiment for 1000 rounds. In this ablation experiment, we study how model make choice within high competitive environment to cerate as much benefit as they can; 
\textbf{Environment Configuration}, we control two environment configuration, initial financial amount and global order number. For each configuration, we sample several stages from low to high to see how agent's behaviors been influenced by the global environment setting.
\textbf{Persona}, we using the model with the best performance to control the agents with persona description in prompts, we sample 20 agents and each persona is allocated to two agents, and we observe how different persona influence the agents behaviors and decision strategies.


\boldstart{Model Competition.}
To intensify inter-agent competition, we constrain each agent to handle at most one order at a time and set the environment's hunger rate to 0.9, ensuring a high demand for delivery. In each experimental session, 24 agents are jointly controlled by 12 different models, where each model governs two agents. These agents actively bid for orders in a shared environment with the goal of maximizing profit. Each session runs for 1000 simulation steps, and results are averaged across three random seeds.

As shown in Figure~\ref{fig:bid(a)}, models exhibit distinct bidding behaviors. Notably, \texttt{Claude-3.7-Sonnet}, \texttt{Gemini-2.5-Flash} and \texttt{Gemini-2.0-Flash} demonstrate broad bid price distributions, indicating a flexible bidding strategy. This flexibility increases their chances of winning orders when in competition with other models. In contrast, models such as \texttt{LLaMA-4-Scout} and \texttt{LLaMA-3.2-11b} tend to use narrower bidding ranges, which limits their competitiveness and results in lower win rates.

Figure~\ref{fig:bid(b)} presents the head-to-head competition outcomes. \texttt{Deepseek-Prover-V2} and \texttt{Qwen3-32B} achieve the highest win rates against other models. This is primarily because they often bid lower prices, making their offers more likely to be accepted by the platform. Conversely, models like \texttt{GPT-4o} and \texttt{LLaMA-3.2-11b} tend to place higher bids, reducing their success rate despite frequent participation. Models such as \texttt{QwQ-32B} and \texttt{GPT-4o-mini} are less active overall, leading to fewer bids and lower order acquisition rates. This inactivity contributes to their diminished final profit, as shown in Table~\ref{tab:main_results}.

\begin{AIbox}{Takeaway: Multi-Agent Competition}
% \texttt{Claude-3.7-Sonnet} and \texttt{Gemini-2.5/2.0-Flash} benefits from wide bid ranges, achieving higher win rates, while \texttt{LLaMA-4-Scout}'s narrow bidding reduces competitiveness.  
Models with flexible bidding strategies, like \texttt{Claude-3.7-Sonnet} and \texttt{Gemini-2.5-Flash}, achieve higher order win rates, while those with narrow or high bids, like \texttt{LLaMA-3.2-11b} and \texttt{GPT-4o}, underperform. Models that bid aggressively, such as \texttt{Deepseek-Prover-V2} and \texttt{Qwen3-32B}, dominate head-to-head competitions, whereas inactive models like \texttt{GPT-4o-mini} fail to secure bids and profits.
\texttt{QwQ} and \texttt{GPT-4o-mini} show minimal bidding activity and weak task participation (Figure~\ref{fig:bid}).
\end{AIbox}

\begin{figure}[ht]
    \vspace*{-5pt}
    \centering
    % \captionsetup{justification=centering, singlelinecheck=false}
    \begin{minipage}{0.55\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/agent_exp2/Combined_Logs_bid_distributions.pdf}
        \subcaption{(a)Bid price distribution by model. The violin plots illustrate the distribution of bid prices generated by each model.Red points indicate bids that were successfully accepted.}
        \label{fig:bid(a)}
    \end{minipage}
    \hfill
    \begin{minipage}{0.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/agent_exp2/Combined_Analysis_head_to_head_matrix.pdf}
        \subcaption{(b)Win-Loss Matrix of Model Competition.}
        \label{fig:bid(b)} 
    \end{minipage}
    % \captionsetup{justification=raggedright} 
    \vspace{-5pt}
    \caption{
        \textbf{Bidding Behavior and Evaluation Results.} 
        \textbf{(a)} %Distribution of bid prices across different models. 
        Lower bid prices may increase the likelihood of being assigned an order, but often come at the cost of reduced profit margins.
        \textbf{(b)} % Head-to-head win-loss matrix summarizing model competition outcomes. 
        Higher values in red represent more wins; lower values in blue indicate more frequent losses in pairs.\vspace{-2pt}
    }\label{fig:bid}
\end{figure}

\boldstart{Environment Configuration.}
We further investigate how different environmental configurations impact agent behavior and overall performance. Specifically, we explore two key factors: the global order availability and the agents’ initial financial endowment. For each factor, we conduct a series of controlled experiments to observe how variations affect agents’ action distributions.

As shown in Figure~\ref{fig:environment}, when the total number of available orders increases, agents tend to perform fewer pickup and delivery actions and instead choose the \texttt{do nothing} action more frequently. 
This suggests that in resource-rich environments, agents are more inclined to conserve energy and avoid unnecessary effort, opting to wait for optimal opportunities rather than actively pursue deliveries. 
Conversely, in low-resource settings, agents are more motivated to engage in delivery tasks to secure profits. 
Additionally, as resource abundance increases, agents demonstrate a higher tendency to initiate and complete shared deliveries, likely as a means to reduce energy costs through collaboration.

Figure~\ref{fig:environment} illustrates the impact of agents’ initial monetary resources. As initial capital increases, agents are less reliant on aggressive bidding and instead prioritize actions such as order pickup. When funds are limited, competition intensifies, leading to more frequent bidding behavior. Furthermore, with sufficient initial capital, agents are more willing to invest in infrastructure, such as purchasing a bike, which enhances their long-term delivery efficiency.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/agent_exp2/legend_horizontal.pdf}
    % \captionsetup{justification=centering, singlelinecheck=false}
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/agent_exp2/all_actions_analysis.pdf}
        \subcaption{(a)Effect of Order Quantity}
        \label{fig:environment(a)}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/agent_exp2/actions_by_money.pdf}
        \subcaption{(b)Effect of Initial Money}
        \label{fig:environment(b)}
    \end{minipage}
    \caption{\textbf{Action Distribution across Environmental Settings.} (a) Shows the change of effect of global order quantity on agent behavior. (b) Shows the effect of initial money on action selection. \label{fig:environment}}
\end{figure}

\begin{AIbox}{Takeaway: Resource and Decision-Making Strategy}
% \begin{itemize}[noitemsep,leftmargin=10pt]
Order resource scarcity increases agent competitiveness and task urgency. Sufficient agent initial money leads to more relaxed, profit-insensitive behavior (Figure~\ref{fig:environment}).
% \end{itemize}
% \vspace{-10pt}
\end{AIbox}

These observations suggest that agents are more competitive and task-driven in resource-constrained environments. In contrast, resource-rich conditions reduce the urgency to complete tasks and generate immediate profits. Importantly, agents are also more likely to engage in actions that involve upfront costs but promise long-term benefits—such as investment and shared delivery—provided they have the financial capacity and enough taken orders to do so.

% \begin{wrapfigure}[15]{r}{0.42\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/agent_exp2/Trait_vs_Win_Rate_Action_Proportion.pdf}
%     \caption{
%         \textbf{Heatmap of Personality Traits on Agent Behavior.} 
%         Pearson correlation b/w Big Five personality traits and agent behaviors.
%     }
%     \label{fig:persona}
    
% \end{wrapfigure}

\begin{figure}
    \centering
    \begin{minipage}{0.44\linewidth}
        \includegraphics[width=\linewidth]{figures/agent_exp2/Trait_vs_Win_Rate_Action_Proportion.pdf}
        \subcaption{(a) Heatmap of Personality Traits on Agent \\ Behavior.}
    \end{minipage}
    \begin{minipage}{0.55\linewidth}
        \vspace{5pt}
        \includegraphics[width=\linewidth]{figures/agent_exp2/Conscientiousness_vs_Bid_Order.pdf}
        \subcaption{(b) Linear Regression Reveals Strong Correlations between Behaviors and Persona Traits.}
        \label{fig:persona(b)}    
    \end{minipage}
    \caption{\textbf{(a) Heatmap of Personality Traits on Agent Behavior.} Pearson correlation b/w Big Five personality traits and agent behaviors.\textbf{(b) Linear Regression Reveals Strong Correlations between Behaviors and Persona Traits.} The results demonstrate that agent behaviors are tightly aligned with their corresponding persona attributes, highlighting the effectiveness of trait-driven behavior modeling. }
    \label{fig:persona}
\end{figure}


\boldstart{Influence of Persona.}
Personality traits significantly affect the decision-making and performance of delivery agents. As shown in Figure~\ref{fig:persona}, agents with higher conscientiousness tend to exhibit a lower frequency of bidding actions, a higher frequency of task-completion actions (e.g., picking up orders), and achieve a higher bid win rate. This suggests that conscientious agents prioritize task completion over strategic competition.
Agents with higher Agreeableness are less likely to remain inactive (i.e., perform "do nothing" actions) and tend to achieve higher bid win rates. Conversely, agents with lower agreeableness display higher inactivity and narrower bidding price ranges, limiting their competitiveness.
Interestingly, agents with higher Openness exhibit reduced engagement in delivery tasks, possibly because they explore competitive or unconventional bidding strategies that divert attention from task execution.




% \begin{figure}[ht]
%     \centering
%     \captionsetup{justification=centering, singlelinecheck=false}
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/persona/Trait_vs_Win_Rate_Action_Proportion.pdf}
%         \subcaption{Heatmap of correlation between big-five persona with behaviors.}
%          \label{fig:persona(a)}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/persona/Conscientiousness_vs_Bid_Order.pdf}
%         \subcaption{Linear regressions reflect behaviors have tight corelation with corresponding persona traits.}
%          \label{fig:persona(b)}        
%     \end{minipage}
%     \captionsetup{justification=raggedright} 
%         \caption{
%     \textbf{Impact of Personality Traits on Agent Behavior.}
%     (a) Heatmap showing Pearson correlation coefficients between Big Five personality traits and key agent behaviors, including bid win rate and action preferences.
%     (b) Linear regression analysis further quantifying persona trait-behavior relation
%     }    \label{fig:persona}
% \end{figure}



\begin{AIbox}{Takeaway: Impact of Persona in Multi-agent Interaction}
Agent personalities shape strategic tendencies: conscientious agents prioritize task fulfillment, while openness and agreeableness modulate competitiveness and inactivity (Figure~\ref{fig:persona}).
\end{AIbox}

\subsubsection{Prompt Design}

\begin{promptbox}{System Prompt of Long-Horizon Delivery Task}
\lstinputlisting[language=Octave,style=mystyle]{prompts/experiment2_system_prompt.py}
\end{promptbox}
\tcbcaption{\textbf{Examples System Prompt of Long-horizon Delivery Task.}
\label{tab:exp2_sys_prompts}}

\begin{promptbox}{User Prompt of Long-Horizon Delivery Task}
\lstinputlisting[language=Octave,style=mystyle]{prompts/experiment2_user_prompt.py}
\end{promptbox}
\tcbcaption{\textbf{Examples User Prompt of Long-horizon Delivery Task.}
\label{tab:exp2_usr_prompts}}

\subsubsection{Chain of Thought Example}
This section, we showcase a representative chain of thought from \texttt{Claude-3.5-Sonnet}. Which shows the model's reasoning process under different circumstances.
\begin{promptbox}{Example Chain of Thought from \texttt{Claude-3.5-Sonnet} on different actions}
\lstinputlisting[language=Octave,style=mystyle]{prompts/case_study2_reasoning.py}
\end{promptbox}
\label{tab:exp2_sys_prompts_non_planner}




==> tables/agent_experiment1_main.tex <==
\begin{table*}[ht]
  \centering
  \caption{\textbf{Performance Comparison across Different Difficulty Levels with Static Obstacles.} 
  SR: Success Rate, CC: Collision Count, CC-S: Collision Count (Success Only), RVR: Red-light Violation Rate, STR: Stuck Rate, NDC: Normalized Decision Count. E: Easy, M: Medium, H: Hard. RVR is not 100\% as agents may happen to cross during green lights. An ablation study with only red lights presented to the agent resulted in a 100\% red-light violation rate, confirming the agent's tendency to ignore red signals when encountered.}
  \vspace*{-5pt}
  \label{tab:baseline-difficulty}
  \scalebox{0.73}{
  \begingroup
  \renewcommand{\arraystretch}{0.9}
  \setlength{\tabcolsep}{2.5pt}
  \hspace*{-5pt}
  \begin{tabular}{lcccccccccccccccc}
    \toprule
    \textbf{Baseline} 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{SR}$\uparrow$} 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{CC}$\downarrow$} 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{CC-S}$\downarrow$} 
    & \cellcolor[HTML]{F2F6FE}\textbf{RVR}$\downarrow$ 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{STR}} 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{NDC}$\downarrow$} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17}
    & E & M & H & E & M & H & E & M & H & H & E & M & H & E & M & H \\
    \midrule
    Rule-based 
    & 66.73 & 63.33 & 40.0 
    & 1.80 & 4.14 & 4.00 
    & 1.55 & 4.74 & 4.67 
    & 0.00
    & 100.00 & 100.00 & 100.00 
    & N/A & N/A & N/A \\
    
    GPT-4o-mini (-8B) 
    & 60.00 & 20.00 & 16.67 
    & 5.97 & 11.13 & 5.33 
    & 4.50 & 7.33 & 6.00 
    & 80.00 
    & 50.00 & 16.77 & 32.00 
    & 3.98 & 2.28 & 4.25 \\
    
    GPT-4o (-200B)
    & 93.33 & 93.33 & \textbf{93.33} 
    & 1.73 & 3.37 & 5.10 
    & 1.64 & 3.46 & 5.07 
    & 67.86 
    & 100.00 & 100.00 & 50.00 
    & 2.22 & 2.48 & 2.32 \\
    
    Claude-3.7-Sonnet (100+B)
    & 86.67 & \textbf{96.67} & \textbf{93.33} 
    & 2.00 & 4.13 & 4.63 
    & 1.81 & 4.10 & 4.50 
    & \textbf{46.43} 
    & 100.00 & 0.00 & 100.00 
    & \textbf{2.07} & \textbf{2.07} & \textbf{2.12} \\
    
    Gemini-2.5-Pro 
    & \textbf{96.70} & 83.30 & 80.0 
    & \textbf{1.50} & \textbf{2.80} & \textbf{3.53}
    & \textbf{1.45} & \textbf{2.76} & \textbf{3.08} 
    & 62.50 
    & 100.00 & 40.00 & 50.00 
    & 2.16 & 2.51 & 2.50 \\
    \bottomrule
  \end{tabular}
  \endgroup}
\vspace*{-10pt}
\end{table*}


==> tables/embodied_multi_agent.tex <==
\begin{table}[t!]
    \centering
    \caption{Experiment results on RoboScape-MRS benchmark.}
    \label{tab:multi-benchmarks}

    % \resizebox{\textwidth}{!}{%
    \footnotesize
    \begin{tabular}{llcc} % Changed to 4 columns: llcc
    \toprule
    \textbf{Models} & \textbf{Method} & CSR\%$\uparrow$ & Task Progress\%$\uparrow$ \\
    \midrule
    \rowcolor{gray!10} \multicolumn{4}{l}{\hspace{1mm}\textit{Proprietary Models}} \\ % Changed to \multicolumn{4}
     GPT-4o & Oracle Planner & 65.00 & 76.90 \\
     Gemini 2.5 Flash & Oracle Planner & 54.55 & 75.84 \\ % Removed extra &
     % GPT-4o & middle-point &  &  &   \\ % Commented out as in original
     GPT-4o & RoCo & 33.33 & 22.93 \\
    \rowcolor{gray!10} \multicolumn{4}{l}{\hspace{1mm}\textit{Open-sourced Models}} \\ % Changed to \multicolumn{4}
    % QwenVL 72B & middle-point & & & &\\ % Commented out as in original
    % InternVL 78B & middle-point & & & & \\ % Commented out as in original
    QwenVL 2.5 72B & RoCo & 11.11 & 35.94 \\ % Removed extra &
    \bottomrule
    \end{tabular}
    % }
\vspace*{-20pt}
\end{table}

==> tables/embodied_single_agent_easy.tex <==
\begin{table}[t!]
    \centering
    \caption{Experimental results on the Multi-modal Robot Navigation (easy task set). The numbers in parentheses indicate the improvement after finetuning.}
    \scriptsize
    \setlength{\tabcolsep}{16pt}
    \label{tab:single-agent-benchmark}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lccc}
    \toprule
    \textbf{Models} & \textbf{SR\%$\uparrow$} & \textbf{Subtask SR\% $\uparrow$} & \textbf{Distance Progress\% $\uparrow$} \\
    \midrule
    \rowcolor{gray!10} \multicolumn{4}{l}{\textit{Proprietary Models}} \\
    GPT-4o & 0 & 33.07 & 15.60 \\
    Gemini 2.5 Flash & 0 & 37.06 & 31.29 \\
    \midrule
    \rowcolor{gray!10} \multicolumn{4}{l}{\textit{Open-sourced Models}} \\
    QwenVL 2.5 7B & 0 & 16.86 & 7.82 \\
    QwenVL 2.5 72B & 0 & 23.80 & 17.50 \\
    Gemma 3 27B & 0 & 15.36 & 6.83 \\
    % InternVL 2.5 8B & 0 & 8.91 & 2e-5 & 3.83 \\
    InternVL 3 78B & 0 & 18.31 & 9.34 \\
    \midrule
    \rowcolor{gray!10} \multicolumn{4}{l}{\textit{Fine-tuned Models}} \\
    QwenVL2.5 7B$_{ft}$  & 4.0 (+4.0) & 52.45 (+35.59) & 53.63 (+45.81) \\
    % InternVL2.5 8B$_{ft}$ &  &  & & \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-15pt}
\end{table}

==> tables/embodied_single_agent_hard.tex <==
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{1pt}
    \caption{Experimental results on the Multi-modal Robot Navigation benchmark (hard task set).}
    \label{tab:single-agent-benchmark}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
    \textbf{Models} & \textbf{SR$\uparrow$} & \textbf{Static Collision$\downarrow$} & \textbf{Dynamic Collision$\downarrow$} & \textbf{Traffic Light Violation$\downarrow$} & \textbf{Subtask SR\%$\uparrow$} & \textbf{Distance Progress\%$\uparrow$} \\
    \midrule
    GPT-4o & 2.08 & 1.92 & 10.37  & 3.02 & 34.38 & 24.83 \\
    Gemini 2.5 Flash & 0 & 3.21 & 4.29 & 7.875 & 32.29 & 29.87 \\
    QwenVL 72B & 0 & 5.0 & 11.73 & 2.86 & 23.86 & 21.97 \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-15pt}
\end{table}

==> tables/physical_ablation.tex <==
\begin{table*}[ht]
  \caption{\textbf{Performance Comparison without Local Action Planner.}
  SR: Success Rate, CC: Collision Count, CC-S: Collision Count (Success Only), DSS: Decision Steps in Success.}
  \label{tab:baseline-non-planner}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lcccccccc}
    \toprule
    \textbf{Baseline}
    & {\cellcolor[HTML]{F2F6FE}\textbf{SR}}$\uparrow$
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{CC}$\downarrow$}
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{CC-S}$\downarrow$}
    & {\cellcolor[HTML]{F2F6FE}\textbf{DSS}}$\downarrow$ \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    & & Building & Object & All & Building & Object & All & \\
    \midrule
    GPT-4o
    & 0
    & 4.5 & 0 & 4.5
    & N/A & N/A & N/A
    & N/A \\

    Claude-3.7-Sonnet
    & 56.67
    & 18.5 & 1.63 & 20.13
    & 11.71 & 2.18 & 13.88
    & \textbf{58.71} \\

    Gemini-2.5-Pro
    & \textbf{60.0}
    & \textbf{15.83} & \textbf{0.4} & \textbf{16.23}
    & \textbf{10.44} & \textbf{0.5} & \textbf{10.94}
    & 68.72 \\
    \bottomrule
  \end{tabular}}
\end{table*}

==> tables/physical_baselines.tex <==
\begin{table*}[ht]
  \centering
  \caption{\textbf{Performance Comparison across Different Difficulty Levels with Static Obstacles.} 
  SR: Success Rate, CC: Collision Count, CC-S: Collision Count (Success Only), RVR: Red-light Violation Rate, STR: Stuck Rate, NDC: Normalized Decision Count. E: Easy, M: Medium, H: Hard. RVR is not 100\% as agents may happen to cross during green lights. An ablation study with only red lights presented to the agent resulted in a 100\% red-light violation rate, confirming the agent's tendency to ignore red signals when encountered.}
  \label{tab:baseline-difficulty}
  \scalebox{0.82}{
  \begingroup
  \renewcommand{\arraystretch}{0.9}
  \setlength{\tabcolsep}{2.5pt}
  \begin{tabular}{lcccccccccccccccc}
    \toprule
    \textbf{Baseline} 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{SR}$\uparrow$} 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{CC}$\downarrow$} 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{CC-S}$\downarrow$} 
    & \cellcolor[HTML]{F2F6FE}\textbf{RVR}$\downarrow$ 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{STR}} 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{NDC}$\downarrow$} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17}
    & E & M & H & E & M & H & E & M & H & H & E & M & H & E & M & H \\
    \midrule
    Rule-based 
    & 66.73 & 63.33 & 40.0 
    & 1.80 & 4.14 & 4.00 
    & 1.55 & 4.74 & 4.67 
    & 0.00
    & 100.00 & 100.00 & 100.00 
    & N/A & N/A & N/A \\
    
    GPT-4o-mini
    & 60.00 & 20.00 & 16.67 
    & 5.97 & 11.13 & 5.33 
    & 4.50 & 7.33 & 6.00 
    & 80.00 
    & 50.00 & 16.77 & 32.00 
    & 3.98 & 2.28 & 4.25 \\
    
    GPT-4o
    & 93.33 & 93.33 & \textbf{93.33} 
    & 1.73 & 3.37 & 5.10 
    & 1.64 & 3.46 & 5.07 
    & 67.86 
    & 100.00 & 100.00 & 50.00 
    & 2.22 & 2.48 & 2.32 \\
    
    Claude-3.7-Sonnet
    & 86.67 & \textbf{96.67} & \textbf{93.33} 
    & 2.00 & 4.13 & 4.63 
    & 1.81 & 4.10 & 4.50 
    & \textbf{46.43} 
    & 100.00 & 0.00 & 100.00 
    & \textbf{2.07} & \textbf{2.07} & \textbf{2.12} \\
    
    Gemini-2.5-Pro 
    & \textbf{96.70} & 83.30 & 80.0 
    & \textbf{1.50} & \textbf{2.80} & \textbf{3.53}
    & \textbf{1.45} & \textbf{2.76} & \textbf{3.08} 
    & 62.50 
    & 100.00 & 40.00 & 50.00 
    & 2.16 & 2.51 & 2.50 \\
    \bottomrule
  \end{tabular}
  \endgroup}
\end{table*}


==> tables/physical_dynamic.tex <==
\begin{table*}[ht]
  \caption{\textbf{Performance Comparison under Dynamic Obstacles.} 
  SR: Success Rate, CC: Collision Count, CC-S: Collision Count (Success Only), NDC: Normalized Decision Count.}
  \label{tab:baseline-dynamic}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{lcccccccc}
    \toprule
    \textbf{Baseline} 
    & {\cellcolor[HTML]{F2F6FE}\textbf{SR}}$\uparrow$ 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{CC}$\downarrow$} 
    & \multicolumn{3}{c}{\cellcolor[HTML]{F2F6FE}\textbf{CC-S}$\downarrow$} 
    & {\cellcolor[HTML]{F2F6FE}\textbf{NDC}$\downarrow$} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    & & Human & Object & All & Human & Object & All & \\
    \midrule
    Rule-based 
    & 80.0 
    & 2.93  & 2.97  & 5.9 
    & 2.54 & 2.83 & 5.38  
    & N/A \\
    
    GPT-4o-mini 
    & 26.67 
    & 1.37 & 3.8 & 5.17 
    & 1.12 & 2.75 & 3.88 
    & 2.43 \\
    
    GPT-4o 
    & 86.67 
    & 1.13 & 2.63 & 3.77 
    & 1.04 & 2.54 & 3.58 
    & 2.3 \\
    
    Claude-3.7-Sonnet 
    & \textbf{93.33} 
    & 1.0 & 2.57 & 3.57 
    & 1.04 & 2.36 & 3.39
    & \textbf{2.27} \\
    
    Gemini-2.5-Pro 
    & 56.67
    & \textbf{0.33} & \textbf{1.6} & \textbf{1.93}
    & \textbf{0.35} & \textbf{1.18} & \textbf{1.53}
    & 2.77 \\
    \bottomrule
  \end{tabular}}
\end{table*}

